Surface Brightness Fluctuations in Two SPT clusters: a Pilot Study

Studies of surface brightness fluctuations in the intracluster medium (ICM) present an indirect probe of turbulent properties such as the turbulent velocities, injection scales, and the slope of the power spectrum of fluctuations towards smaller scales. With the advancement of Sunyaev-Zel'dovich (SZ) studies and surveys relative to X-ray observations, we seek to investigate surface brightness fluctuations in a sample of SPT-SZ clusters which also have archival \textit{XMM-Newton} data. Here we present a pilot study of two typical clusters in that sample: SPT-CLJ0232-4421 and SPT-CLJ0638-5358. We infer injection scales larger than 500 kpc in both clusters and Mach numbers $\approx 0.5$ in SPT-CLJ0232-4421 and Mach numbers $\approx 0.6 - 1.6$ in SPT-CLJ0638-5358, which has a known shock. We find hydrostatic bias values for $M_{500}$ less than 0.2 for SPT-CLJ0232-4421 and less than 0.1 for SPT-CLJ0638-5358. These results show the importance to assess its quantitative values via a detailed multiwavelength approach and suggest that the drivers of turbulence may occur at quite larger scales.

==> BackupHydBiases_27Aug2023.tex <==
\begin{table}[!h] 
   \centering  
   \begin{tabular}{c | c c c c | c c c c} 
                  & \multicolumn{4}{c}{SPT-CLJ0232-4421} & \multicolumn{4}{c}{SPT-CLJ0638-5358} \\
    $R_{\rm ell}$ & $a/b$ & $\theta_R$ & Ring & $-b_{\mathcal{M}}$ & $a/b$ & $\theta_R$ & Ring & $-b_{\mathcal{M}}$ \\ 
   \hline 

\multirow{2}{*}{$\phi = \sqrt{3}$} & \multirow{2}{*}{1} & \multirow{2}{*}{0} & Ring 1 & $0.21 \pm 0.39$ & 
\multirow{2}{*}{1} & \multirow{2}{*}{0} & Ring 1 & $-0.20 \pm 0.23$ \\ 
 & & & Ring 2 & $0.25 \pm 0.17$  & & & Ring 2 & $0.03 \pm 0.38$ \\ 

\multirow{2}{*}{$\phi = (1 + \sqrt{5})/2$} & \multirow{2}{*}{1} & \multirow{2}{*}{0} & Ring 1 & $0.34 \pm 0.20$ &
\multirow{2}{*}{1} & \multirow{2}{*}{0} & Ring 1 & $-0.42 \pm 0.65$ \\ 
 & & & Ring 2 & $0.13 \pm 0.10$  & & & Ring 2 & $0.02 \pm 0.73$ \\ 

\multirow{2}{*}{$\phi = \sqrt{2}$} & \multirow{2}{*}{1} & \multirow{2}{*}{0} & Ring 1 & -- & \multirow{2}{*}{1} & \multirow{2}{*}{0} & Ring 1 & -- \\ 
 & & & Ring 2 & --  & & & Ring 2 & -- \\ 

\multirow{2}{*}{Peak} & \multirow{2}{*}{1} & \multirow{2}{*}{0} & Ring 1 & -- & 
\multirow{2}{*}{1} & \multirow{2}{*}{0} & Ring 1 & $-0.21 \pm 0.34$ \\ 
 & & & Ring 2 & --  & & & Ring 2 & $0.10 \pm 0.38$ \\ 

\hline 

\multirow{2}{*}{1.0} & \multirow{2}{*}{1.14} & \multirow{2}{*}{140} & Ring 1 & $0.28 \pm 0.19$ & 
\multirow{2}{*}{1.15} & \multirow{2}{*}{164} & Ring 1 & $-0.22 \pm 0.34$ \\ 
 & & & Ring 2 & $0.07 \pm 0.08$   & & & Ring 2 & $0.05 \pm 0.45$ \\ 

\multirow{2}{*}{1.5} & \multirow{2}{*}{1.07} & \multirow{2}{*}{141} & Ring 1 & $0.28 \pm 0.19$ & 
\multirow{2}{*}{1.17} & \multirow{2}{*}{158} & Ring 1 & $-0.20 \pm 0.30$ \\ 
 & & & Ring 2 & $0.09 \pm 0.08$   & & & Ring 2 & $0.06 \pm 0.40$ \\ 

\multirow{2}{*}{2.0} & \multirow{2}{*}{1.06} & \multirow{2}{*}{139} & Ring 1 & $0.30 \pm 0.19$  & 
\multirow{2}{*}{1.17} & \multirow{2}{*}{150} & Ring 1 & $-0.22 \pm 0.30$ \\
 & & & Ring 2 & $0.10 \pm 0.08$   & & & Ring 2 & $0.04 \pm 0.43$ \\ 

\multirow{2}{*}{2.5} & \multirow{2}{*}{1.05} & \multirow{2}{*}{123} & Ring 1 & $0.30 \pm 0.20$ & 
\multirow{2}{*}{1.18} & \multirow{2}{*}{145} & Ring 1 & $-0.20 \pm 0.29$ \\ 
 & & & Ring 2 & $0.11 \pm 0.09$   & & & Ring 2 & $0.06 \pm 0.39$ \\ 

\multirow{2}{*}{3.0} & \multirow{2}{*}{1.07} & \multirow{2}{*}{101} & Ring 1 & $0.27 \pm 0.18$ & 
\multirow{2}{*}{1.19} & \multirow{2}{*}{142} & Ring 1 & $-0.20 \pm 0.29$ \\ 
 & & & Ring 2 & $0.11 \pm 0.08$   & & & Ring 2 & $0.06 \pm 0.39$ \\ 

\multirow{2}{*}{3.5} & \multirow{2}{*}{1.09} & \multirow{2}{*}{95} & Ring 1 & $0.27 \pm 0.19$ & 
\multirow{2}{*}{1.20} & \multirow{2}{*}{146} & Ring 1 & $-0.19 \pm 0.28$ \\  
 & & & Ring 2 & $0.10 \pm 0.08$   & & & Ring 2 & $0.06 \pm 0.38$ \\ 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{2}{*}{4.0} & \multirow{2}{*}{1.11} & \multirow{2}{*}{92} & Ring 1 & $0.27 \pm 0.19$ & 
\multirow{2}{*}{1.21} & \multirow{2}{*}{145} & Ring 1 & $-0.17 \pm 0.27$ \\
 & & & Ring 2 & $0.09 \pm 0.08$   & & & Ring 2 & $0.06 \pm 0.37$ \\ 

\multirow{2}{*}{4.5} & \multirow{2}{*}{1.12} & \multirow{2}{*}{91} & Ring 1 & $0.23 \pm 0.18$ & 
\multirow{2}{*}{1.21} & \multirow{2}{*}{146} & Ring 1 & $-0.16 \pm 0.27$ \\
 & & & Ring 2 & $0.09 \pm 0.08$   & & & Ring 2 & $0.08 \pm 0.36$ \\ 

\multirow{2}{*}{5.0} & \multirow{2}{*}{1.11} & \multirow{2}{*}{95} & Ring 1 & $0.26 \pm 0.18$ & 
\multirow{2}{*}{1.21} & \multirow{2}{*}{144} & Ring 1 & $-0.18 \pm 0.29$ \\ 
 & & & Ring 2 & $0.09 \pm 0.08$   & & & Ring 2 & $0.06 \pm 0.38$ \\ 

\multirow{2}{*}{5.5} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & 
\multirow{2}{*}{--} & \multirow{2}{*}{1.20} & \multirow{2}{*}{144} & Ring 1 & $-0.18 \pm 0.29$ \\ 
& & & &  & & & Ring 2 & $0.06 \pm 0.38$ \\ 

\multirow{2}{*}{6.0} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & 
\multirow{2}{*}{--} & \multirow{2}{*}{1.19} & \multirow{2}{*}{142} & Ring 1 & $-0.16 \pm 0.30$ \\ 
& & & &  & & & Ring 2 & $0.09 \pm 0.38$ \\ 

\hline
   \end{tabular} 
   \caption{Hydrostatic mass biases as derived for different ellipticities. $R_{\rm ell}$ is the radius at which ellipticity parameters are determined (as in Figure~\ref{fig:EllipticityParams}). $a/b$ is then the axis ratio and $\theta_R$ is the rotation angle (in degrees). The first four rows show results from circular cases and either different ring extents or different center; entries for $\phi = (1 + \sqrt{5})/2$ are the reprint of the hydrostatic biases in Table~\ref{tbl:bms}. All numbers for elliptical fits use $\phi = (1 + \sqrt{5})/2$ to define the ring extents. Empty entries for SPT-CLJ0638-5358 arise from a lack of nodes (in Ring 2) about $2\sigma$; empty entries for SPT-CLJ0232-4421 reflect that $R_{500} = 5.^{\prime}3$ and thus elliptical parameters are not pursued beyond $R_{500}$.}
   \label{tbl:bms_ell_both}
\end{table} 

==> BackupLitMasses.tex <==
\begin{table}[!h] 
   \centering  
   \begin{tabular}{c c c c | c c} 
 Facility & Work & Cosmology & Quantity & SPT-CLJ0232-4421 & SPT-CLJ0638-5358 \\ 
\hline 
\multirow{3}{*}{SPT} & Bleem15 & Flat$^{a}$ + $\sigma_8 = 0.8$ & $M_{500}$  & $ 12.01_{-1.80}^{+1.80}$ & $ 12.01_{-1.81}^{+1.81}$ \\ 
 & Bocquet19 & Flat$^{a}$ + $\sigma_8 = 0.8$ & $M_{500}$  & $ 11.30_{-1.36}^{+1.11}$ & $ 11.29_{-1.36}^{+1.10}$ \\ 
 & Bulbul19 & de Haan (2016) & $M_{500}$  & $ 9.45_{-1.10}^{+1.16}$ & $ 9.42_{-1.09}^{+1.18}$ \\ 
 & Bulbul19 & X-ray stuff & $M_{\text{gas}}$  & $1.67_{-0.08}^{+0.08} $ & $0.97_{-0.21}^{+0.21}$ \\ 
 \hline
\multirow{3}{*}{ACT} & Hilton21 & Flat$^{a}$ & $M_{500,uncorr}$  & $ 10.12_{-1.75}^{+2.12}$  & $ 10.47_{-1.91}^{+2.33}$ \\ 
 & Hilton21 & Flat$^{a}$ & $M_{500,c}$  & $ 8.73_{-1.43}^{+1.71}$  & $ 8.91_{-1.53}^{+1.85}$ \\ 
 & Hilton21 & Flat$^{a}$ & $M_{500,cal}$  & $ 12.30_{-1.43}^{+2.70}$  & $ 12.54_{-1.53}^{+2.88}$ \\ 
 \hline
ComPRASS & & & $M_{500}$  & $ 7.82_{-0.96}^{+0.90}$ & $ 8.61_{-0.67}^{+0.64}$ \\ 
MCXC & Delete & This? & $M_{500}$  & $ 6.13$ & $ 6.88$ \\ 
REFLEX & Mantz+ 2010 & Mantz+ 2010 & $M_{500}$ & $12.7 \pm 2.5$ & $10.3 \pm 1.4$ \\
Reichardt+ 2011 & Zhang+ 2008 & Mantz+ 2010 & $M_{500}$ & $8.4 \pm 2.5$ & $10.3 \pm 1.4$ \\
          & (XMM + ROSAT) & (CXO + ROSAT) & $M_{X,1}$ &  $7.54 \pm 2.20$ & -- \\
          & (XMM + ROSAT) & (CXO + ROSAT) & $M_{X,2}$ &  $8.39 \pm 2.42$ & -- \\
          & (XMM + ROSAT) & (CXO + ROSAT) & $M_{\text{gas,}500}$ & $0.89\pm 0.09$ & $1.18 \pm 0.13$ \\
Lensing & PSZ-MCMF & Fox+ 2022 & &  $7.54_{-0.32}^{+0.33}$  & $8.41$ \\
Lensing & Klein+ 2019 & & $M_{500,1}$ & $5.13_{-1.69}^{+1.94}$ & \\
Lensing & Klein+ 2019 & & $M_{500,2}$ & $4.08_{-1.31}^{+1.67}$ & \\
My Numbers & Assuming & A10 is & gospel & $8.36 \pm 0.05 $ & $7.70 \pm 0.05$ \\
\hline
\multirow{3}{*}{PSZ} & Salvati22 & Whatever fit & $M_{500,free}$  & $10.35_{-2.63}^{+2.72}$  & $ 9.24_{-2.40}^{+2.44}$ \\ 
 & Salvati22 & Planck & $M_{500,fixed}$  & $ 11.16_{-1.14}^{+1.52}$  & $ 9.51_{-1.11}^{+1.81}$ \\ 
 & Planck XXVII (2015) & Planck & $M_{500}$ & 7.54 & 6.83
   \end{tabular} 
   \caption{$^{a}$ $\Lambda$CDM with $\Omega_m = 0.3$, $\Omega_{\Lambda} = 0.7$, and $H_0 = 70$ km/s/Mpc}  
   \label{tbl:lit_masses}
\end{table} 


==> BadHydrostaticBiasTable.tex <==
\begin{table}[!h] 
   \centering  
   \begin{tabular}{c c | c c c} 
    & & $-b_{\mathcal{M}}$ & $d \ln P / d \ln r$ & $d \ln \mathcal{M}_{\text{3D}}/ d \ln r$ \\ 
   \hline 
   \multirow{2}{*}{SPT-CLJ0232-4421} & Ring 1 & $0.23 \pm 0.25$ & $0.27 \pm 0.30$ & \multirow{2}{*}{$0.25 \pm 0.35$} \\ 
    & Ring 2 &  $0.17 \pm 0.13$ &  $-3.42 \pm 0.09$ &  \\ 
    \hline
    \multirow{2}{*}{SPT-CLJ0638-5358} & Ring 1 & $-0.42 \pm 0.40$ & $-1.22 \pm 0.01$ & \multirow{2}{*}{$1.51 \pm 0.53$} \\
     & Ring 2 & $0.01 \pm 0.48$ & $-3.04 \pm 0.11$ &  \\
   \end{tabular} 
   \caption{Derived hydrostatic biases and logarithmic slopes of which the biases are functions.}  
   \label{tbl:bms}
\end{table} 

%%% $-0.918 \pm 0.382 logarithmic Mach slope for 0232-4421
%%% $0.610 \pm 0.409$ logarithmic Mach slope for 0638-5358

==> EllipticalHydBiases.tex <==
\begin{table}[!h] 
   \centering  
   \begin{tabular}{c c | c c c c c c c c c c c c} 
     &         & $R_{\rm ell}$: & 0.0 & 1.0 & 1.5 & 2.0 & 2.5 & 3.0 & 3.5 & 4.0 & 4.5 & 5.0 & 5.5 & 6.0 \\
     & cluster &  & & & & & & & & & & & & \\
     \multirow{4}{*}{SPT-CLJ0232-4421} & $a/b$ & 1.0 & 1.14 & 1.07 & 1.06 & 1.05 & 1.07 & 1.09 & 1.11 & 1.21 & 1.11 & & \\
                                 & $\theta_R$  & 0.0 & 140  & 141  & 139  & 123  & 101  & 95   & 92   & 91   & 95   & & \\
     & $-b_{\mathcal{M},1}$ & $0.14 \pm 0.13$ & $0.14 \pm 0.12$ & $0.13 \pm 0.11$ & $0.08 \pm 0.19$ & $0.13 \pm 0.13$ & 
     $0.08 \pm 0.21$ & $0.07 \pm 0.22$ & $0.11 \pm 0.11$ & $0.08 \pm 0.10$ & $0.11 \pm 0.11$ \\
     & $-b_{\mathcal{M},2}$ & $0.14 \pm 0.07$ & $0.08 \pm 0.06$ & $0.11 \pm 0.06$ & $0.13 \pm 0.10$ & $0.12 \pm 0.07$ &
     $0.12 \pm 0.11$ & $0.12 \pm 0.12$ & $0.10 \pm 0.06$ & $0.10 \pm 0.05$ & $0.10 \pm 0.06$ \\
      \hline
      \multirow{4}{*}{SPT-CLJ0638-5358} & $a/b$ & 1.0 & 1.15 & 1.17 & 1.17 & 1.18 & 1.19 & 1.20 & 1.21 & 1.21 & 1.21 & 1.20 & 1.19 \\
                                 & $\theta_R$   & 0.0 & 164  & 158  & 150  & 145  & 142  & 146  & 145  & 146  & 144  & 144  & 142  \\
      & $-b_{\mathcal{M},1}$ & $-0.48 \pm 0.35$ & $-0.24 \pm 0.18$ & $-0.22 \pm 0.16$  & $-0.25 \pm 0.15$ & $-0.21 \pm 0.15$ & $-0.22 \pm 0.15$ & $-0.21 \pm 0.15$ &
      $-0.18 \pm 0.16$ & $-0.17 \pm 0.16$ & $-0.18 \pm 0.17$ & $-0.20 \pm 0.15$ & $-0.18 \pm 0.17$  \\
      & $-b_{\mathcal{M},2}$ & $0.03 \pm 0.40$ &  $0.06 \pm 0.26$ & $0.07 \pm 0.23$ & $0.04 \pm 0.23$ & $0.07 \pm 0.22$ & $0.06 \pm 0.22$ & $0.06 \pm 0.22$ 
      & $0.08 \pm 0.22$ & $0.09 \pm 0.21$ & $0.09 \pm 0.23$ & $0.08 \pm 0.22$ & $0.09 \pm 0.23$ \\
      \hline
   \end{tabular} 
   \caption{Filler Caption}  
   \label{tbl:bms_ells}
\end{table} 

==> HydrostaticBias_Ell_0232.tex <==
\begin{table}[!h] 
   \centering  
   \begin{tabular}{c c c | c c} 
    & $-b_{\mathcal{M},\text{comb}}$ & $d \ln P / d \ln r$ \\ 
   \hline 
   Ring 1 & 1.0 & 1.14 & 140 & $0.14 \pm 0.12$ \\ 
   Ring 2 & 1.0 & 1.14 & 140 & $0.08 \pm 0.06$ \\ 
   \hline
   Ring 1 & 1.5 & 1.07 & 141 & $0.13 \pm 0.11$ \\ 
   Ring 2 & 1.5 & 1.07 & 141 & $0.11 \pm 0.06$ \\ 
   \hline
    Ring 1 & 2.0 & 1.06 & 139 & $0.08 \pm 0.19$ \\ 
    Ring 2 & 2.0 & 1.06 & 139 & $0.13 \pm 0.10$ \\ 
   \hline 
   Ring 1 & 2.5 & 1.05 & 123 & $0.13 \pm 0.13$ \\ 
   Ring 2 & 2.5 & 1.05 & 123 & $0.12 \pm 0.07$ \\ 
   \hline
   Ring 1 & 3.0 & 1.07 & 101 & $0.08 \pm 0.21$ \\ 
   Ring 2 & 3.0 & 1.07 & 101 & $0.12 \pm 0.11$ \\ 
   \hline 
   Ring 1 & 3.5 & 1.09 & 95 & $0.07 \pm 0.22$ \\ 
   Ring 2 & 3.5 & 1.09 & 95 & $0.12 \pm 0.12$ \\  
   \hline 
   Ring 1 & 4.0 & 1.11 & 92 & $0.11 \pm 0.11$ \\ 
   Ring 2 & 4.0 & 1.11 & 92 & $0.10 \pm 0.06$ \\    
    \hline 
   Ring 1 & 4.5 & 1.12 & 91 & $0.08 \pm 0.10$ \\ 
   Ring 2 & 4.5 & 1.12 & 91 & $0.10 \pm 0.05$ \\ 
    \hline 
   Ring 1 & 5.0 & 1.11 & 95 & $0.11 \pm 0.11$ \\ 
   Ring 2 & 5.0 & 1.11 & 95 & $0.10 \pm 0.06$ \\ 
   \end{tabular} 
   \caption{Filler Caption}  
   \label{tbl:bms_ell_0232}
\end{table} 


==> KeySpectralQuantities_Old.tex <==
\begin{table}[!h] 
   \centering  
   \begin{tabular}{c c c | c c c c} 
    Cluster & Dataset & Ring & A$_{\text{3D}} (k_{\text{peak}})$ & $\sigma_{\text{3D}}$ & $k_{\text{peak}} $ & $\lambda_{\text{peak}}$ \\
    & & & & & (arcmin$^{-1}$) & (kpc) \\ 
   \hline 
   \multirow{2}{*}{SPT-CLJ0232-4421} & X-ray & Ring 1 & $0.13 \pm 0.02$ & $0.15 \pm 0.02$ & 0.49 & 516 \\ 
   & X-ray & Ring 2 & $0.16 \pm 0.07$ & $0.10 \pm 0.16$ & 0.30 & 837 \\ 
   \hline
   \multirow{3}{*}{SPT-CLJ0638-5358} & X-ray & Ring 1 & $0.15 \pm 0.03$ & $0.15 \pm 0.15$ & 0.27 & 807 \\ 
    & SZ & Ring 1 & $0.23 \pm 0.11$ & $0.13 \pm 0.36$ & 0.16 & 1380 \\
    & X-ray & Ring 2 & $0.40 \pm 0.12$ & $0.26 \pm 0.44$ & 0.27 & 807 \\ 
    \hline
   \end{tabular} 
   \caption{Key values from amplitude or power spectra.}  
   \label{tbl:ps_products}
\end{table} 


==> MachNumberTable.tex <==
\begin{table}[!h] 
   \centering  
   \begin{tabular}{c c c | c c} 
    Cluster & Dataset & Ring & $\mathcal{M}_{\text{3D,peak}}$ & $\mathcal{M}_{\text{3D,int}}$ \\ 
   \hline 
   \multirow{2}{*}{SPT-CLJ0232-4421} & X-ray & Ring 1 & $0.51 \pm 0.06$ & 0.32 \\ 
   & X-ray & Ring 2 & $0.63 \pm 0.26$ & 0.21 \\ 
   \hline
    \multirow{3}{*}{SPT-CLJ0638-5358} & X-ray & Ring 1 & $0.64 \pm 0.03$ & 0.33 \\ 
     & SZ & Ring 1 & $0.56 \pm 0.26$ & 0.31 \\ 
    & X-ray & Ring 2 & $1.60 \pm 0.46$ & 0.55 \\ 
   \hline
   \end{tabular} 
   \caption{Derived Mach numbers }  
   \label{tbl:mach_numbers}
\end{table} 


==> OldHydrostaticMassBiases_August2023.tex <==
\begin{table}[!h] 
   \centering  
   \begin{tabular}{c c | c c c} 

      & & $-b_{\mathcal{M},\text{peak}}$ & $-b_{\mathcal{M},\text{int}}$ & $-b_{\mathcal{M},\text{comb}}$ \\ 
   \hline 
   \multirow{2}{*}{SPT-CLJ0232-4421} & Ring 1 & $0.01 \pm 0.25$ & $0.13 \pm 0.16$ & $0.08 \pm 0.30$ \\ 
    & Ring 2 & $0.15 \pm 0.12$ & $0.03 \pm 0.06$ & $0.09 \pm 0.15$ \\ 
    \hline
    \multirow{2}{*}{SPT-CLJ0638-5358} & Ring 1 & $-0.43 \pm 0.41$ & $-0.02 \pm 0.17$ & $-0.16 \pm 0.42$ \\ 
    & Ring 2 & $0.01 \pm 0.48$ & $0.07 \pm 0.20$ & $0.08 \pm 0.54$ \\ 
    
   % & & $-b_{\mathcal{M}}$ & $d \ln P / d \ln r$ & $d \ln \mathcal{M}_{\text{3D}}/ d \ln r$ \\ 
   %\hline 
   %\multirow{2}{*}{SPT-CLJ0232-4421} & Ring 1 & $0.05 \pm 0.19$ & $-0.75 \pm 0.01$ & \multirow{2}{*}{$0.08 \pm 1.22$} \\ 
   % & Ring 2 &  $0.06 \pm 0.10$ &  $-3.42 \pm 0.09$ &  \\ 
   % \hline
   % \multirow{2}{*}{SPT-CLJ0638-5358} & Ring 1 & $-0.17 \pm 0.37$ & $-1.22 \pm 0.01$ & \multirow{2}{*}{$1.19 \pm 1.00$} \\
   %  & Ring 2 & $0.13 \pm 0.37$ & $-3.04 \pm 0.11$ &  \\
   \end{tabular} 
   \caption{Derived hydrostatic biases and logarithmic slopes of which the biases are functions.}  
   \label{tbl:bms}
\end{table} 

==> OldMachAndBiases_0638Slices.tex <==
\begin{table}[!h] 
   \centering  
   \begin{tabular}{c c | c c | c c} 
             &        & \multicolumn{2}{c}{Ring 1} & \multicolumn{2}{c}{Ring 2} \\
    Quadrant & $\phi$ & $\mathcal{M}_{\text{3D,peak}}$ & $-b_{\mathcal{M}}$ & $\mathcal{M}$ & $-b_{\mathcal{M}}$ \\ 
    \hline
    \multirow{3}{*}{Q1} & $\sqrt{3}$ & $0.50 \pm 0.04$ & $-0.26 \pm 0.23$ & $1.37 \pm 0.57$ & $0.03 \pm 0.40$ \\
                & $(1 + \sqrt{5})/2$ & $0.60 \pm 0.06$ & -- & -- & -- \\
                        & $\sqrt{2}$ & $0.67 \pm 0.04$ & -- & -- & -- \\
    \hline
    \multirow{3}{*}{Q2} & $\sqrt{3}$ & $0.62 \pm 0.10$ & $-0.47 \pm 0.47$ & $1.71 \pm 0.57$ & $0.06 \pm 0.51$ \\
                & $(1 + \sqrt{5})/2$ & $0.67 \pm 0.04$ & $-0.41 \pm 0.51$ & $1.58 \pm 0.62$ & $0.15 \pm 0.42$ \\
                        & $\sqrt{2}$ & $0.86 \pm 0.07$ & -- & -- & -- \\              
    \hline
    \multirow{3}{*}{Q3} & $\sqrt{3}$ & $0.36 \pm 0.07$ & $-0.09 \pm 0.09$ & $0.87 \pm 0.30$ &  $0.06 \pm 0.15$ \\
                & $(1 + \sqrt{5})/2$ & $0.44 \pm 0.07$ & -- & -- & -- \\
                        & $\sqrt{2}$ & $0.53 \pm 0.11$ & -- & -- & -- \\
    \hline
    \multirow{3}{*}{Q4} & $\sqrt{3}$ & $0.77 \pm 0.10$ & $-0.79 \pm 0.78$ & $2.01 \pm 0.47$ &  $0.16 \pm 0.41$ \\
                & $(1 + \sqrt{5})/2$ & $0.75 \pm 0.14$ & $-0.78 \pm 1.00$ & $1.94 \pm 0.56$ & $0.05 \pm 0.66$ \\
                        & $\sqrt{2}$ & $0.87 \pm 0.08$ & $0.02 \pm 0.35$ & $1.22 \pm 0.35$ & $0.33 \pm 0.18$ \\
    \hline
    \end{tabular} 
   \caption{Mach numbers and corresponding hydrostatic mass biases; empty fields arise due to a lack of points in our amplitude spectra above $2\sigma$.}  
   \label{tbl:bms_quads_0638}
\end{table} 

==> OldMachTable_August2023.tex <==
\begin{table}[!h] 
   \centering  
   \begin{tabular}{c c c | c c c} 
    Cluster & Dataset & Ring & $\mathcal{M}_{\text{3D,peak}}$ & $\mathcal{M}_{\text{3D,int}}$ & $\mathcal{M}_{\text{3D,comb}}$ \\ 
   \hline 
   \multirow{2}{*}{SPT-CLJ0232-4421} & X-ray & Ring 1 & $0.51 \pm 0.06$ & $0.32 \pm 0.02$ & $0.41 \pm 0.09 \pm 0.02$ \\ 
   & X-ray & Ring 2 & $0.63 \pm 0.26$ & $0.21 \pm 0.19$ & $0.42 \pm 0.21 \pm 0.15$ \\ 
   \hline
    \multirow{3}{*}{SPT-CLJ0638-5358} & X-ray & Ring 1 & $0.60 \pm 0.10$ &  $0.31 \pm 0.18$ & $0.46 \pm 0.14 \pm 0.09$ \\ 
     & SZ & Ring 1 & $0.56 \pm 0.26$ & $0.31 \pm 0.50$ & $0.44 \pm 0.12 \pm 0.23$ \\ 
    & X-ray & Ring 2 & $1.58 \pm 0.46$ & $0.54 \pm 0.53$ & $1.06 \pm 0.52 \pm 0.35$ \\ 
   \hline
   \end{tabular} 
   \caption{Derived Mach numbers.}  
   \label{tbl:mach_numbers}
\end{table} 


==> OldMassTable.tex <==
\begin{table}[!h] 
   \centering  
   \begin{tabular}{c c | c c} 
 Work & Quantity & SPT-CLJ0232-4421 & SPT-CLJ0638-5358 \\ 
\hline 
SPT & $M_{500}$  & $ 11.30_{-1.36}^{+1.11}$ & $ 11.29_{-1.36}^{+1.10}$ \\ 
\hline
\multirow{3}{*}{ACT} & $M_{500,uncorr}$  & $ 10.12_{-1.75}^{+2.12}$  & $ 10.47_{-1.91}^{+2.33}$ \\ 
 & $M_{500,c}$  & $ 8.73_{-1.43}^{+1.71}$  & $ 8.91_{-1.53}^{+1.85}$ \\ 
 & $M_{500,cal}$  & $ 12.30_{-1.43}^{+2.70}$  & $ 12.54_{-1.53}^{+2.88}$ \\ 
 \hline
ComPRASS & $M_{500}$ & $ 7.82_{-0.96}^{+0.90}$ & $8.61_{-0.67}^{+0.64}$ \\ 
MCXC & $M_{500}$ & 6.13 & $6.88$ \\ 
\hline
\multirow{2}{*}{PSZ} & $M_{500,free}$  & $ 7.24_{-5.40}^{+9.15}$  & $ 6.47_{-4.79}^{+8.17}$ \\ 
 & $M_{500,fixed}$  & $ 7.81_{-7.01}^{+8.87}$  & $ 6.66_{-5.88}^{+7.92}$ \\ 
 \hline
   \end{tabular} 
   \caption{Filler Caption}  
   \label{tbl:ps_products}
\end{table} 

==> Olhd_BigVerticalHydrBiases.tex <==
\begin{table}[!h] 
   \centering  
   \begin{tabular}{c | c c c c | c c c c} 
                  & \multicolumn{4}{c}{SPT-CLJ0232-4421} & \multicolumn{4}{c}{SPT-CLJ0638-5358} \\
    $R_{\rm ell}$ & $a/b$ & $\theta_R$ & Ring & $-b_{\mathcal{M}}$ & $a/b$ & $\theta_R$ & Ring & $-b_{\mathcal{M}}$ \\ 
   \hline 

\multirow{2}{*}{$\phi = \sqrt{3}$} & \multirow{2}{*}{1} & \multirow{2}{*}{0} & Ring 1 & $-0.11 \pm 0.20$ & \multirow{2}{*}{1} & \multirow{2}{*}{0} & Ring 1 & $-0.20 \pm 0.14$ \\ 
 & & & Ring 2 & $0.17 \pm 0.09$  & & & Ring 2 & $0.02 \pm 0.25$ \\ 

\multirow{2}{*}{$\phi = (1 + \sqrt{5})/2$} & \multirow{2}{*}{1} & \multirow{2}{*}{0} & Ring 1 & $0.01 \pm 0.25$ & \multirow{2}{*}{1} & \multirow{2}{*}{0} & Ring 1 & $-0.42 \pm 0.40$ \\ 
 & & & Ring 2 & $0.15 \pm 0.12$  & & & Ring 2 & $0.01 \pm 0.48$ \\ 

\multirow{2}{*}{$\phi = \sqrt{2}$} & \multirow{2}{*}{1} & \multirow{2}{*}{0} & Ring 1 & $0.11 \pm 0.20$ & \multirow{2}{*}{1} & \multirow{2}{*}{0} & Ring 1 & -- \\ 
 & & & Ring 2 & $0.13 \pm 0.09$  & & & Ring 2 & -- \\ 

\multirow{2}{*}{Peak} & \multirow{2}{*}{1} & \multirow{2}{*}{0} & Ring 1 & $0.24 \pm 0.16$ & \multirow{2}{*}{1} & \multirow{2}{*}{0} & Ring 1 & $-0.20 \pm 0.21$ \\ 
 & & & Ring 2 & $0.11 \pm 0.08$  & & & Ring 2 & $0.10 \pm 0.24$ \\ 

\hline 

\multirow{2}{*}{1.0} & \multirow{2}{*}{1.14} & \multirow{2}{*}{140} & Ring 1 & $0.10 \pm 0.12$ & \multirow{2}{*}{1.15} & \multirow{2}{*}{164} & Ring 1 & $-0.22 \pm 0.21$ \\ 
 & & & Ring 2 & $0.08 \pm 0.06$   & & & Ring 2 & $0.05 \pm 0.29$ \\ 

\multirow{2}{*}{1.5} & \multirow{2}{*}{1.07} & \multirow{2}{*}{141} & Ring 1 & $0.08 \pm 0.12$ & \multirow{2}{*}{1.17} & \multirow{2}{*}{158} & Ring 1 & $-0.20 \pm 0.19$ \\ 
 & & & Ring 2 & $0.10 \pm 0.06$   & & & Ring 2 & $0.06 \pm 0.26$ \\ 

\multirow{2}{*}{2.0} & \multirow{2}{*}{1.06} & \multirow{2}{*}{139} & Ring 1 & $0.04 \pm 0.20$  & \multirow{2}{*}{1.17} & \multirow{2}{*}{150} & Ring 1 & $-0.22 \pm 0.19$ \\
 & & & Ring 2 & $0.12 \pm 0.10$   & & & Ring 2 & $0.03 \pm 0.28$ \\ 

\multirow{2}{*}{2.5} & \multirow{2}{*}{1.05} & \multirow{2}{*}{123} & Ring 1 & $0.09 \pm 0.14$ & \multirow{2}{*}{1.18} & \multirow{2}{*}{145} & Ring 1 & $-0.19 \pm 0.18$ \\ 
 & & & Ring 2 & $0.11 \pm 0.07$   & & & Ring 2 & $0.06 \pm 0.25$ \\ 

\multirow{2}{*}{3.0} & \multirow{2}{*}{1.07} & \multirow{2}{*}{101} & Ring 1 & $0.05 \pm 0.21$ & \multirow{2}{*}{1.19} & \multirow{2}{*}{142} & Ring 1 & $-0.20 \pm 0.18$ \\ 
 & & & Ring 2 & $0.11 \pm 0.11$   & & & Ring 2 & $0.05 \pm 0.25$ \\ 

\multirow{2}{*}{3.5} & \multirow{2}{*}{1.09} & \multirow{2}{*}{95} & Ring 1 & $0.06 \pm 0.12$ & \multirow{2}{*}{1.20} & \multirow{2}{*}{146} & Ring 1 & $-0.18 \pm 0.17$ \\  
 & & & Ring 2 & $0.10 \pm 0.06$   & & & Ring 2 & $0.05 \pm 0.24$ \\ 

\multirow{2}{*}{4.0} & \multirow{2}{*}{1.11} & \multirow{2}{*}{92} & Ring 1 & $0.07 \pm 0.12$ & \multirow{2}{*}{1.21} & \multirow{2}{*}{145} & Ring 1 & $-0.17 \pm 0.17$ \\
 & & & Ring 2 & $0.09 \pm 0.06$   & & & Ring 2 & $0.06 \pm 0.24$ \\ 

\multirow{2}{*}{4.5} & \multirow{2}{*}{1.12} & \multirow{2}{*}{91} & Ring 1 & $0.05 \pm 0.11$ & \multirow{2}{*}{1.21} & \multirow{2}{*}{146} & Ring 1 & $-0.15 \pm 0.17$ \\
 & & & Ring 2 & $0.09 \pm 0.06$   & & & Ring 2 & $0.08 \pm 0.23$ \\ 

\multirow{2}{*}{5.0} & \multirow{2}{*}{1.11} & \multirow{2}{*}{95} & Ring 1 & $0.07 \pm 0.11$ & \multirow{2}{*}{1.21} & \multirow{2}{*}{144} & Ring 1 & $-0.16 \pm 0.18$ \\ 
 & & & Ring 2 & $0.09 \pm 0.06$   & & & Ring 2 & $0.07 \pm 0.25$ \\ 

\multirow{2}{*}{5.5} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{1.20} & \multirow{2}{*}{144} & Ring 1 & $-0.18 \pm 0.18$ \\ 
& & & &  & & & Ring 2 & $0.06 \pm 0.25$ \\ 

\multirow{2}{*}{6.0} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{1.19} & \multirow{2}{*}{142} & Ring 1 & $-0.16 \pm 0.18$ \\ 
& & & &  & & & Ring 2 & $0.08 \pm 0.24$ \\ 

\hline
   \end{tabular} 
   \caption{Hydrostatic mass biases as derived for different ellipticities. $R_{\rm ell}$ is the radius at which ellipticity parameters are determined (as in Figure~\ref{fig:EllipticityParams}). $a/b$ is then the axis ratio and $\theta_R$ is the rotation angle (in degrees). The first four rows show results from circular cases and either different ring extents or different center; entries for $\phi = (1 + \sqrt{5})/2$ are the reprint of the hydrostatic biases in Table~\ref{tbl:bms}. All numbers for elliptical fits use $\phi = (1 + \sqrt{5})/2$ to define the ring extents. Empty entries for SPT-CLJ0638-5358 arise from a lack of nodes (in Ring 2) about $2\sigma$; empty entries for SPT-CLJ0232-4421 reflect that $R_{500} = 5.^{\prime}3$ and thus elliptical parameters are not pursued beyond $R_{500}$.}
   \label{tbl:bms_ell_both}
\end{table} 

==> SPT-CLJ0638-5358_ProductsFrom3DXRspectra_within3p6-6p3__BCGum-OneCXB-Sliced_2023-06-12-slices.tex <==
\begin{table}[!h] 
   \centering  
   \begin{tabular}{c | c c c c} 
    & & A$_{\text{3D}}$ & $\sigma_{\text{3D}}$ & $k_{\text{peak}}(^{\prime^{-1}}) $ & $\lambda_{\text{peak}}$ (kpc) \\ 
   \hline 
   Ring 1 & Slice 1 & $0.19 \pm 0.02$ & 0.18 & 0.27 & 806.62 \\ 
   Ring 1 & Slice 2 & $0.22 \pm 0.04$ & 0.25 & 0.47 & 471.46 \\ 
   Ring 1 & Slice 3 & $0.13 \pm 0.02$ & 0.12 & 0.27 & 806.62 \\ 
   Ring 1 & Slice 4 & $0.25 \pm 0.03$ & 1.84 & 0.47 & 471.46 \\ 
   Ring 2 & Slice 1 & $0.27 \pm 0.16$ & 0.16 & 0.27 & 806.62 \\ 
   Ring 2 & Slice 2 & $0.39 \pm 0.12$ & 0.21 & 0.27 & 806.62 \\ 
   Ring 2 & Slice 3 & $0.17 \pm 0.09$ & 0.13 & 0.16 & 1380.03 \\ 
   Ring 2 & Slice 4 & $0.42 \pm 0.11$ & 0.28 & 0.27 & 806.62 \\ 
   \end{tabular} 
   \caption{Filler Caption}  
   \label{tbl:ps_products}
\end{table} 


==> SPT-CLJ0638-5358_ProductsFrom3DXRspectra_within3p6-6p3__BCGum-OneCXB-Sliced_2023-06-12-slices_MachNumbers.tex <==
\begin{table}[!h] 
   \centering  
   \begin{tabular}{c c | c c} 
    & & $\mathcal{M}_{\text{3D,peak}}$ & $\mathcal{M}_{\text{3D,int}}$ \\ 
   \hline 
   Ring 1 & Slice 1 & $0.76 \pm 0.07$ & 0.36 \\ 
   Ring 1 & Slice 2 & $0.90 \pm 0.17$ & 0.51 \\ 
   Ring 1 & Slice 3 & $0.53 \pm 0.08$ & 0.26 \\ 
   Ring 1 & Slice 4 & $1.02 \pm 0.14$ & 3.82 \\ 
   Ring 2 & Slice 1 & $1.07 \pm 0.66$ & 0.33 \\ 
   Ring 2 & Slice 2 & $1.54 \pm 0.49$ & 0.44 \\ 
   Ring 2 & Slice 3 & $0.67 \pm 0.35$ & 0.26 \\ 
   Ring 2 & Slice 4 & $1.67 \pm 0.45$ & 0.59 \\ 
   \end{tabular} 
   \caption{SPT-CLJ0638-5358 -- Old Mach numbers}  
   \label{tbl:OldMachNumbers-0638}
\end{table} 


==> SPT-CLJ0638-5358_ProductsFrom3DXRspectra_within3p9-6p3__noMask-OneCXB_v2-Sliced_2023-06-17-slices.tex <==
\begin{table}[!h] 
   \centering  
   \begin{tabular}{c c | c c c c} 
    & & A$_{\text{3D}}$ & $\sigma_{\text{3D}}$ & $k_{\text{peak}}(^{\prime^{-1}}) $ & $\lambda_{\text{peak}}$ (kpc) \\ 
   \hline 
   Ring 1 & Slice 1 & $0.20 \pm 0.02$ & 0.18 & 0.27 & 806.62 \\ 
   Ring 1 & Slice 2 & $0.23 \pm 0.05$ & 0.25 & 0.47 & 471.46 \\ 
   Ring 1 & Slice 3 & $0.15 \pm 0.03$ & 0.12 & 0.27 & 806.62 \\ 
   Ring 1 & Slice 4 & $0.28 \pm 0.05$ & 0.86 & 0.47 & 471.46 \\ 
   Ring 2 & Slice 1 & $0.00 \pm 0.29$ & 0.10 & 0.47 & 471.46 \\ 
   Ring 2 & Slice 2 & $0.37 \pm 0.14$ & 0.20 & 0.27 & 806.62 \\ 
   Ring 2 & Slice 3 & $0.00 \pm 0.00$ & 0.09 & 0.47 & 471.46 \\ 
   Ring 2 & Slice 4 & $0.40 \pm 0.12$ & 0.27 & 0.27 & 806.62 \\ 
   \end{tabular} 
   \caption{Filler Caption}  
   \label{tbl:ps_products}
\end{table} 


==> SPT-CLJ0638-5358_ProductsFrom3DXRspectra_within3p9-6p3__noMask-OneCXB_v2-Sliced_2023-06-17-slices_MachNumbers.tex <==
\begin{table}[!h] 
   \centering  
   \begin{tabular}{c c | c c} 
    & & $\mathcal{M}_{\text{3D,peak}}$ & $\mathcal{M}_{\text{3D,int}}$ \\ 
   \hline 
   Ring 1 & Slice 1 & $0.81 \pm 0.08$ & 0.38 \\ 
   Ring 1 & Slice 2 & $0.93 \pm 0.19$ & 0.51 \\ 
   Ring 1 & Slice 3 & $0.59 \pm 0.11$ & 0.25 \\ 
   Ring 1 & Slice 4 & $1.10 \pm 0.18$ & 1.79 \\ 
   Ring 2 & Slice 1 & $0.00 \pm 1.14$ & 0.20 \\ 
   Ring 2 & Slice 2 & $1.46 \pm 0.56$ & 0.42 \\ 
   Ring 2 & Slice 3 & $0.00 \pm 0.00$ & 0.18 \\ 
   Ring 2 & Slice 4 & $1.60 \pm 0.48$ & 0.56 \\ 
   \end{tabular} 
   \caption{SPT-CLJ0638-5358 Mach numbers}  
   \label{tbl:MachNumbers0638}
\end{table} 


==> VerticalbM_Ell.tex <==
\begin{table}[!h] 
   \centering  
   \begin{tabular}{c | c c c c | c c c c} 
                  & \multicolumn{4}{c}{SPT-CLJ0232-4421} & \multicolumn{4}{c}{SPT-CLJ0638-5358} \\
    $R_{\rm ell}$ & $a/b$ & $\theta_R$ & Ring & $-b_{\mathcal{M}}$ & $a/b$ & $\theta_R$ & Ring & $-b_{\mathcal{M}}$ \\ 
   \hline 

 \multirow{2}{*}{$\phi = \sqrt{3}$} & \multirow{2}{*}{1} & \multirow{2}{*}{0} & Ring 1 & $-0.10 \pm 0.43$ & \multirow{2}{*}{1} & \multirow{2}{*}{0} & Ring 1 & $-0.20 \pm 0.10$ \\
 & & & Ring 2 & $0.19 \pm 0.13$ & & & Ring 2 & $0.00 \pm 0.21$ \\ 
 
\multirow{2}{*}{$\phi = (1 + \sqrt{5})/2$} & \multirow{2}{*}{1} & \multirow{2}{*}{0} & Ring 1 & $0.06 \pm 0.24$ & \multirow{2}{*}{1} & \multirow{2}{*}{0} & Ring 1 & $-0.44 \pm 0.35$ \\ 
 & & & Ring 2 & $0.16 \pm 0.02$ & & & Ring 2 & $0.07 \pm 0.35$ \\ 

  \multirow{2}{*}{$\phi = \sqrt{2}$} & \multirow{2}{*}{1} & \multirow{2}{*}{0} & Ring 1 &  $0.16 \pm 0.33$ & \multirow{2}{*}{1} & \multirow{2}{*}{0} & Ring 1 & $0.20 \pm 0.28$ \\
  & & & Ring 2 & $0.15 \pm 0.17$ & & & Ring 2 & $0.15 \pm 0.22$ \\
 
 \multirow{2}{*}{Peak} & \multirow{2}{*}{1} & \multirow{2}{*}{0} & Ring 1 & $0.27 \pm 0.14$ & \multirow{2}{*}{1} & \multirow{2}{*}{0} & Ring 1 & $-0.20 \pm 0.17$ \\ 
 & & & Ring 2 & $0.12 \pm 0.08$ & & & Ring 2 & $0.10 \pm 0.21$ \\ 
 
 \hline

\multirow{2}{*}{1.0} & \multirow{2}{*}{1.14} & \multirow{2}{*}{140} & Ring 1 & $0.14 \pm 0.12$ & \multirow{2}{*}{1.15} & \multirow{2}{*}{164} & Ring 1 & $-0.24 \pm 0.18$ \\ 
 & & & Ring 2 & $0.08 \pm 0.06$ & & & Ring 2 & $0.06 \pm 0.26$ \\ 
 
\multirow{2}{*}{1.5} & \multirow{2}{*}{1.07} & \multirow{2}{*}{141} & Ring 1 & $0.13 \pm 0.11$ & \multirow{2}{*}{1.17} & \multirow{2}{*}{158} & Ring 1 & $-0.22 \pm 0.16$ \\ 
 & & & Ring 2 & $0.11 \pm 0.06$ & & & Ring 2 & $0.07 \pm 0.23$ \\ 
    
\multirow{2}{*}{2.0} & \multirow{2}{*}{1.06} & \multirow{2}{*}{139} & Ring 1 & $0.08 \pm 0.19$ & \multirow{2}{*}{1.17} & \multirow{2}{*}{150} & Ring 1 & $-0.25 \pm 0.15$ \\ 
 & & & Ring 2 & $0.13 \pm 0.10$ & & & Ring 2 & $0.04 \pm 0.23$ \\ 
    
\multirow{2}{*}{2.5} & \multirow{2}{*}{1.05} & \multirow{2}{*}{123} & Ring 1 & $0.13 \pm 0.13$ & \multirow{2}{*}{1.18} & \multirow{2}{*}{145} & Ring 1 & $-0.21 \pm 0.15$ \\
 & & & Ring 2 & $0.12 \pm 0.07$ & & & Ring 2 & $0.07 \pm 0.22$ \\ 
    
\multirow{2}{*}{3.0} & \multirow{2}{*}{1.07} & \multirow{2}{*}{101} & Ring 1 & $0.08 \pm 0.21$ & \multirow{2}{*}{1.19} & \multirow{2}{*}{142} & Ring 1 & $-0.22 \pm 0.15$ \\ 
 & & & Ring 2 & $0.12 \pm 0.11$ & & & Ring 2 & $0.06 \pm 0.22$ \\ 
 
\multirow{2}{*}{3.5} & \multirow{2}{*}{1.09} & \multirow{2}{*}{95} & Ring 1 & $0.07 \pm 0.22$ & \multirow{2}{*}{1.20} & \multirow{2}{*}{146} & Ring 1 & $-0.21 \pm 0.15$ \\ 
 & & & Ring 2 & $0.12 \pm 0.12$  & & & Ring 2 & $0.06 \pm 0.22$ \\ 
   
\multirow{2}{*}{4.0} & \multirow{2}{*}{1.11} & \multirow{2}{*}{92} & Ring 1 & $0.11 \pm 0.11$ & \multirow{2}{*}{1.21} & \multirow{2}{*}{145} & Ring 1 & $-0.18 \pm 0.16$ \\ 
 & & & Ring 2 & $0.10 \pm 0.06$ & & & Ring 2 & $0.08 \pm 0.22$ \\ 
    
\multirow{2}{*}{4.5} & \multirow{2}{*}{1.12} & \multirow{2}{*}{91} & Ring 1 & $0.08 \pm 0.10$ & \multirow{2}{*}{1.21} & \multirow{2}{*}{146} & Ring 1 & $-0.17 \pm 0.16$ \\ 
 & & & Ring 2 & $0.10 \pm 0.05$ & & & Ring 2 & $0.09 \pm 0.21$ \\ 
    
\multirow{2}{*}{5.0} & \multirow{2}{*}{1.11} & \multirow{2}{*}{95} & Ring 1 & $0.11 \pm 0.11$  & \multirow{2}{*}{1.21} & \multirow{2}{*}{144} & Ring 1 & $-0.18 \pm 0.17$ \\ 
 & & & Ring 2 & $0.10 \pm 0.06$ & & & Ring 2 & $0.09 \pm 0.23$ \\ 
\multirow{2}{*}{5.5}  & & & & & \multirow{2}{*}{1.20} & \multirow{2}{*}{144} & Ring 1 & $-0.20 \pm 0.15$ \\ 
 & & & & & & & Ring 2 & $0.08 \pm 0.22$ \\ 
\multirow{2}{*}{6.0} & & & & & \multirow{2}{*}{1.19} & \multirow{2}{*}{142} & Ring 1 & $-0.18 \pm 0.17$ \\ 
 & & & & & & & Ring 2 & $0.09 \pm 0.23$ \\ 
 \hline
   \end{tabular} 
   \caption{Hydrostatic mass biases as derived for different ellipticities. $R_{\rm ell}$ is the radius at which ellipticity parameters are determined (as in Figure~\ref{fig:EllipticityParams}). $a/b$ is then the axis ratio and $\theta_R$ is the rotation angle (in degrees). The rows corresponding to $R_{\rm ell} = 0$ are the reprint of the hydrostatic biases in Table~\ref{tbl:bms}}  
   \label{tbl:bms_ell_both}
\end{table} 
